Connecting quantum circuit amplitudes and matrix permanents through polynomials

In this paper, we strengthen the connection between qubit-based quantum circuits and photonic quantum computation. Within the framework of circuit-based quantum computation, the sum-over-paths interpretation of quantum probability amplitudes leads to the emergence of sums of exponentiated polynomials. In contrast, the matrix permanent is a combinatorial object that plays a crucial role in photonic by describing the probability amplitudes of linear optical computations. To connect the two, we introduce a general method to encode an $\mathbb F_2$-valued polynomial with complex coefficients into a graph, such that the permanent of the resulting graph's adjacency matrix corresponds directly to the amplitude associated the polynomial in the sum-over-path framework. This connection allows one to express quantum amplitudes arising from qubit-based circuits as permanents, which can naturally be estimated on a photonic quantum device.

==> sections/appendices/framework.tex <==
\section{Framework} \label{app:framework}

In his work, Rudolph \cite{rudolph_simple_2009} proposes a method to encode the
amplitudes of quantum circuits built upon the gates Hadamard and Toffoli as
permanents of the adjacency matrices associated to graphs -- or more loosely,
permanents of graphs. To achieve this, the circuit is first associated to a low
degree polynomial $f$ over $\mathbb F_2$ and each clause of that polynomial is
associated with a graph gadget. The individual gadgets are then linked together
with cycles representing the variables they share to form the final graph.
Reading the permanent of a graph as the sum of the weights of its cycle covers
allows one to interpret the permanent as a sum over the assignments of the
variables. Computing the graph permanent of $G$ therefore \emph{bruteforces} the
computation of the exponential sum
\begin{equation}
    \per G = \sum_{\substack{\x \in \{0, 1\}^{n}}}(-1)^{f(\x)},
\end{equation}
by computing the value of each cycle cover. The weight of a \emph{valid} cycle
cover corresponds to one of the $(-1)^{f(\x)}$ using the following rule
mentioned in the main text: in a particular cycle cover, the absence of a cycle
corresponding to a variable corresponds to the fact that the variable is
assigned the value 1, and its presence corresponds to its assignment to 0.
However, notice that not all cycle covers correspond to a valid assignment of
the variables, see example in \autoref{fig:validInvalidCoverApp}. The bold blue
edges represent the cycles associated to variables.
% \begin{figure}[hbtp!]
%     \centering%
%     \begin{subfigure}[t]{.45\textwidth}%
%         \centering%
%         \input{img/valid_cycle_cover.tex}
%         \caption{\emph{Valid} cycle cover. Say vertex 1 is connected to the
%         variable $x$ and 2 to $y$, then the cycle cover assigns $x = 0$ and $y =
%         1$, and the contribution of the gadget is $(-1)^{xy} = 1$.}
%         \label{fig:validCoverApp}
%     \end{subfigure}\hfill%
%     \begin{subfigure}[t]{.45\textwidth}
%         \centering
%         \input{img/invalid_cycle_cover.tex}
%         \caption{\emph{Invalid} cycle cover. The overall contribution of such
%         covers must be zero. See example of
%         \autoref{fig:quadraticGadgetsCrossingPaths}.}
%         \label{fig:invalidCoverApp}
%     \end{subfigure}
%     \caption{Illustrative example of the gadget representing the quadratic clauses
%     of the polynomial from \cite{rudolph_simple_2009}. Example of a cycle cover
%     corresponding to a valid assignment of the variable in \autoref{fig:validCoverApp}
%     and an invalid one in \autoref{fig:invalidCoverApp}.}
%     \label{fig:validInvalidCoverApp}
% \end{figure}

The covers that traverse a cycle corresponding to a variable cannot be
associated with a consistent assignment of that variable, therefore their
contributions should interfere destructively and sum up to zero. An example of
such cancellation is given in \autoref{fig:quadraticGadgetsCrossingPaths}. The
properties of the polynomial are direct consequence of its encoding. It is a
polynomial of degree 3, in which each variable that appears in a cubic clause
must then appear in two quadratic clauses. This property is ensured by
construction: each target of the Toffoli gates must be followed by a pair of
Hadamard gates hence the degree is bounded. This additional, necessary structure
ensures that quadratic clause gadgets suffice to \emph{force} an external edge
which is incident to the cubic clause gadget to leave via the same vertex it
entered. Therefore, a simpler cubic clause gadget can be used, as it does not
have to satisfy these constraints on the cycle covers, and no gadget for clauses
of degree higher than 3 is needed. The major drawback is that the pair of
Hadamard gates, used to bound the degree, is required even when the degree does
not have to be bounded. This is the case for IQP circuits, which are the focus
of this work \cite{montanaro_quantum_2017}.


\begin{figure}[hbtp!]
    \centering
    \begin{subfigure}{.45\textwidth}
        \centering
        \input{img/quadratic_gadget_crossing_paths_1.tex}
        \caption{Part of a crossing cycle.}
        \label{fig:crossPath1}
    \end{subfigure}\hfill%
    \begin{subfigure}{.45\textwidth}
        \centering
        \input{img/quadratic_gadget_crossing_paths_2.tex}
        \caption{Part of another crossing cycle.}
        \label{fig:crossPath2}
    \end{subfigure}
    \caption{Illustrative example of the gadget representing the quadratic clauses
    of the polynomial from \cite{rudolph_simple_2009}. The blue edges correspond to
    cycles representing the variables. The gadget design must be so that each
    crossing path can be paired with another with contribution of opposite sign to
    the cycle cover in a way which causes the necessary cancellation. In this
    instance, the contribution depicted in \autoref{fig:crossPath1} is cancelled by
    the one shown in \autoref{fig:crossPath2}.}
    \label{fig:quadraticGadgetsCrossingPaths}
\end{figure}



==> sections/appendices/method.tex <==
\section{Gate gadget design}\label{app:gateGadgetDesign}

This section is intended to explain how the methods in \cite{rudolph_simple_2009} can be
formalized and how the finding of a gate-gadget can be systematized. The two
\autoref{ob:nonzero,ob:zero} of \autoref{sec:method} are suitably described
mathematically employing computational algebraic geometry techniques. Given a gadget, we
denote by \emph{outer vertices} all the vertices connected to the rest of the
graph, \ie the vertices associated to the variables, and by \emph{inner
vertices} the vertices only connected within the gadget. The inner vertices will
account for additional degrees of freedom in the weights the cycle covers of the
gadget so that all the constraints (see the rest of the section) are satisfied.
For instance, in
\autoref{fig:validInvalidCover,fig:quadraticGadgetsCrossingPaths}, the
\emph{outer vertices} are the vertices $1$ and $2$, and the vertex $3$ is the
only \emph{inner vertex}. We now describe how \autoref{ob:nonzero,ob:zero}
translate into a system of equations, so that a solution to that system is the
gadget we seek. Say one wants to represent a clause of degree $d$, and requires
$k$ inner degrees of freedom, \ie $k$ additional inner vertices that allow to
have \emph{enough} possible paths to fulfill all conditions. The gadget is a
graph with $k+d$ vertices, $d$ of which are outer vertices and $k$ are inner
vertices. The adjacency matrix of the graph is thus of order $k+d$.
% ($|\OO| = d$ and $|\II| = k$.)

\paragraph{Nonzero contribution. (\autoref{ob:nonzero})} We consider a cycle
cover consistent with an assignment of the variables. In order to satisfy the
\autoref{ob:nonzero}, one has to make sure that the weight of a valid cycle
cover of a gadget is equal to the amplitude as described in
\autoref{eq:amplitudeBalancedGate}, according to the assignment of the variables
connected to that gadget. Recall that each boolean variable $x_i$ is associated
to a cycle in the graph, and that if that particular cycle is present in the
cycle cover then this matches the variable assignment $x_i = 0$ and if it is not
then $x_i = 1$. For a gadget representing a clause of degree $d$ we write $\s$
the bit-string representing one of the $2^d$ possible assignments of the
variables. The polynomial equation associated to $\s$ is the permanent of the
graph induced by all inner vertices and the outer vertices that are indexed by 1
in $\s$, or equivalently the permanent of the adjacency matrix where all rows
and columns indexed by 0 in $\s$ are removed. The polynomial must equate to $1$
whenever $f = 0$, and $e^{i \theta}$ for a parameter $\theta \in [0, 2\pi]$
otherwise. This naturally induces $2^d$ equations.

\paragraph{Zero contribution. (\autoref{ob:zero})} We consider a cycle cover
inconsistent with an assignment of the variables. When looking only at a
traversed gadget, we call a cycle cover with a path crossing a gadget entering
in vertex $x$ and exiting in vertex $y$ a \emph{partial cycle cover}, and we
write it $x \toc y$. A path $x \to y$ (that can traverse any inner vertices and
possibly outer vertices) is called a \emph{crossing path} of the partial cycle
cover. \autoref{fig:quadraticGadgetsCrossingPaths} actually illustrates two
partial cycle covers of the form $1\toc 2$. The term \emph{partial cycle cover}
may be misleading; the cycle covers are indeed actual cycle covers, but they are
partial from the perspective of a single gadget, in the sense that they do not
cover the whole gadget. Incidentally, the cycle covers that correspond to a
valid assignment of the variables are those that are not \emph{partial} for any
gadget. For a partial cycle cover $x \toc y$, we denote by $\omega(x \toc y)$
the weight of the cycle cover, \ie the product of the weights of the edges
involved in it. A gadget $A = (V_A, E_A)$ is valid if the sum of the weights of
all its partial cycle covers is zero. Let us denote by $\OO_A \subseteq V_A$ the
set of outer vertices of $A$. From the perspective of a whole graph $G=(V_G,
E_G)$ (in which $A$ is included, so that $V_A \subset V_G$ and $E_A \subset
V_G$), the contribution of the partial cycle covers of $A$ is zero if and only
\begin{equation}\label{eq:zeroContribution}
    \begin{aligned}
        \sum_{(x, y) \in \OO_A \times \OO_A}
            \left(
                \sum_{c \in \{x\toc y\}} \omega(c) \per{G_c},
            \right) = 0
    \end{aligned}
\end{equation}
where $G_c$ is some graph depending on the cover $c$ we describe in the next
paragraph. Designing a valid therefore implies to find the proper weights of the
edges such that the above condition is satisfied. On the one hand, imposing
$\omega(c) = 0$ for all partial cycle cover $c$ of the gadget is too
restrictive, as it would not imply that the gadget is not a connected graph, but
also that none of the nonzero contribution can be fulfilled. On the other hand,
we will show that we cannot consider all partial cycle covers at once and simply
imposing ${\sum_c\omega(c) = 0}$, as this would not imply
\autoref{eq:zeroContribution} in the general case. We denote by $\mathscr P(S)$
the power set of any set $S$. Observe that for a particular partial cycle cover
$x\toc y$ traversing the set ${o \in \mathscr P(\OO_A - \{\{x\}, \{y\}\})}$ of
outer vertices of $A$, $G_c$ is, in all generality, composed of a component
connected to both $x$ and $y$ which we write $G_{o,(xy)}$ and a disconnected
component $\overline{G_o}$ (which is connected to all outer vertices not in $o$,
thus disconnected from the partial cycle cover). We virtually disconnect $G_{o,
(xy)}$ from $x$ and $y$, add the edge $x \to y$ of weight one and denote this
newly constructed graph $G_{o,x\to y}$, so that the contribution of the rest of
the graph, when considering the partial cycle cover $x \toc y$ that traverses
the vertices of $o$, is $\per{G_{o, x\to y}} \per{\overline{G_o}}$. In that
regard, \autoref{eq:zeroContribution} rewrites
% \begin{widetext}
\begin{equation}\label{eq:traversedGadgetContribution}
    \begin{aligned}

        \sum_{(x, y) \in \OO_A \times \OO_A}
            \left(
                \sum_{o \in \mathscr P (\OO_A - \{\{x\}, \{y\}\} )}
                \per{G_{o,x\to y}}
                \per{\overline{G_o}}
                \left(
                    \sum_{
                        \substack{
                            c' \in \{x\toc y\}\\
                            \text{$c'$ traverses all}\\
                            \text{vertices of $o$}}
                    } \omega(c')
                \right)
            \right) = 0.
    \end{aligned}
\end{equation}
% \end{widetext}
This is illustrated in \autoref{fig:generalizedCrossingPath}, in which we are
interested of the contribution once the pair of vertices is chosen to be $(1, 2)$.
Let us describe the contribution of $\CC_1$: $G_{\{1, 2\}, 1\to 2}$ is ``Graph
1'' disconnected from the rest and with the additional edge $1 \to 2$ is  and
``Graph 2'' is $\overline{G_{\{1, 2\}}}$. During the process of designing a
gadget, the only control one has is on the weights $\omega(c)$ for $c = \CC_1,
\CC_2$, as all the other terms of \autoref{eq:traversedGadgetContribution}
depend on a specific instance. But still, one must ens that
\autoref{eq:traversedGadgetContribution} holds. Hence, in order to design a
clause gadget whose supposedly zero contributions are effectively zero, one must
ensure that, for all $(x, y) \in \OO_A \times \OO_A$ and for all $o \in \mathscr
P (\OO_A - \{\{x\}, \{y\}\} )$, the following holds
\begin{equation}\label{eq:isZeroAndMustBeZero}
    \sum_{
        \substack{
            c \in \{x\toc y\}\\
            \text{$c$ traverses all}\\
            \text{vertices of $o$}}
    } \omega(c) = 0 .
\end{equation}
Applying \autoref{eq:isZeroAndMustBeZero} to the example of
\autoref{fig:generalizedCrossingPath} yields
\begin{equation}
        \sum_{c \in \CC_1} \omega(c) = \sum_{c \in \CC_2} \omega(c) = 0.
\end{equation}
Consequently, a gadget $A$ might require several inner vertices to have enough
degrees of freedom (the supplementary nodes and the weights on their connected
edges) to satisfy \autoref{eq:isZeroAndMustBeZero}. Note that it does not show
that grouping the partial cycle cover with respect to the set of outer vertices
they traverse is the most efficient way to design a gadget, in the sense that
there might be a way to group them in bigger groups, therefore lowering the
number of inner vertices required. However,
\autoref{eq:traversedGadgetContribution} seems to indicate that this choice is
optimal as we only have a local control on each contribution (the
$\omega(c)$'s).


\begin{figure}[hbtp!]
    \centering
    \input{img/crossing_path_condition.tex}
    \caption{The purple rectangle represents a gadget with three outer vertices,
    the inner vertices are not shown. Crossing paths of partial cycle cover must
    enter and exit through the same pair of vertices and traverse exactly the
    same set of outer vertices for them to cancel each other. In the depicted
    case, the set of paths that cancel each other out must enter and exit
    through vertices 1 and 2 and traverse the same set of outer vertices, \ie
    the partial cycle cover $\CC_1$ cannot cancel the contributions of $\CC_2$.}
\label{fig:generalizedCrossingPath}
\end{figure}


The construction of the system of equations for the zero contributions is
slightly more involved than the nonzero case. Given two outer vertices $x$ and $y$ in $\OO_A$, we want
that all the partial cycle covers $x \toc y$ have zero contribution. In order to
write the constraints on the contributions of all partial covers $x \toc y$  --
comprising the paths $x \to y$ --  as permanent equations we use the following
trick. Given $x$ and $y$, we set to 0 all the entries of the $y$-th row of the
adjacency matrix, apart from the $x$-th entry that we set to 1. This way, all
edges exiting $y$ are removed and an artificial edge $y \to x$ is created, so
that all crossing paths $x \to y$ are transformed into cycles. As a result, the
permanent of the remaining graph is exactly the sum of all the contributions of
the partial covers $x \toc y$. Recall that we grouped the paths $x \toc y$
according to the set of outer vertices they traverse, hence this procedure is
applied \emph{separately} to such set. From a pair $(x, y)$ and a set of outer
vertices, the procedure generates a single polynomial. We repeat this procedure
for all pairs of outer vertices, and we obtain a system of $2^{d-2}d(d-1)$
equations. The overall procedure to generate the system of equations is
summarized in \autoref{alg:generation}, and the resulting system of polynomial
equations is characterized in the following \autoref{pr:characterization}.
Observe that the algorithm does no computation, \ie no permanent is actually
computed, but the variables are symbolically manipulated to write down
polynomials.


\begin{proposition}[Characterisation of the system of equations]
    \label{pr:characterization}
    Let $A$ be the adjacency matrix of a gadget representing a clause of degree
    $d$ with $k$ inner degrees of freedom. Then, the \autoref{alg:generation}
    generates a system of $\ 2^d\left(d(d-1)2^{-2} + 1\right)$ multilinear
    polynomial equations in $(k+d)^2$ variables. It runs in time
    $\Theta(2^d)$.
\end{proposition}


\begin{algorithm}[h!t]
    \caption{Procedure for the generation of the constraints of the $P_i(\theta)$ gates}
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
    \Input{\begin{itemize}
        \setlength\itemsep{.1em}
        \item $d$ the degree of the clause
        \item $k$ the number of inner degrees of freedom
        \item $f_{\UU}$ the polynomial associated to the gate $\UU$
    \end{itemize}}
    \Output{The family of polynomial equations associated to the input parameters.}
    \Begin{
     Let $F$ be the list of polynomials.\\
     Let $A := (x_{ij})_{1 \leq i, j \leq k+d}$ be the symbolic adjacency matrix
     of the gadget.\\
     Let $\OO$ (resp. $\II$) be the set of outer (resp. inner) vertices indexes. \\
    \For{\textbf{all} $d$-bits strings $\s$}{
         Let $\OO_{\s}$ be the subset of $\OO$ where we keep only the indexes indexed by 1 in $\s$.\\
         $F \leftarrow F \cup \per{A_{\OO_{\s}\cup \II}} - e^{i \theta f_{\UU}(\s)}$.
    }%\EndFor
    \For{\textbf{all} $(x, y) \in \OO \times \OO$ s.t. $x \neq y$}{
        \For {$\bs s \in \mathscr P(\OO - \{\{x\},\{y\}\})$}{
             $A_{\{x, y\} \cup \bs s \cup \II} $ be the graph induced by the vertices $x, y$, those in $\bs s$ and the inner vertices.\\
             Set the row representing $y$ to zero, apart from the $x$-th entry that is set to 1 in $A_{\{x, y\} \cup \bs s \cup \II}$.\\
             $F \leftarrow F \cup \per{A_{\{x, y\} \cup \bs s \cup \II}}$
        }%\EndFor
    }%\EndFor
    \Return $F$
    }
    \label{alg:generation}
\end{algorithm}
A drawback of \autoref{alg:generation} is its
verbosity. Therefore, before computing the reduced Gröbner basis of a system of
polynomial equations, we advise using Laplace's expansion formula along a row,
which reads for the $i$-th
\begin{equation}
\per{A} = \sum_{j=1}^n a_{i,j} \per{A_{\bar{i},\bar{j}}},
\end{equation}
where $A_{\bar{i},\bar{j}}$ is the submatrix of $A$ obtained by removing the
$i$-th row and the $j$-th column. This relies on the fact that
\autoref{alg:generation} sets the value of many submatrix permanents
\smash{$\per{A_{\bar{i},\bar{j}}}$}, which can then be substituted in the rest
of the system. If a numerical solution is sought, one can use homotopy
continuation \cite{chen_homotopy_2015}, as many computer algebra system do not
implement solution finding from the reduced Gröbner basis over the complex
numbers when the variety is not zero-dimensional \cite{berthomieu_msolve_2021,
demin_groebner_2023}. Finding a solution, that is, a clause gadget, takes
exponential time \cite{bardet_complexity_2015}, but it is a
\emph{compute-once-and-store-forever} operation which becomes negligible in the
long run.

==> sections/benchmark.tex <==
\section{Estimation of quantum circuits amplitudes in practice}\label{sec:benchmark}


This task is applied to IQP circuits simply because they come with hardness
results, yet, they are highly structured and combinatorial arguments are rather
straightforward. Nonetheless, such an analysis could be perform on other family
of circuit, albeit seemingly much harder without structure.


Using  \cite{hoeffding_probability_1963}, we can estimate the error in the
estimate one computes from sampling. Hence, for a fixed error in the estimate,
not only it is possible to express the number of samples required to achieve
that error, but also the number of samples required in one scheme as a function
of the number of samples required in the other. With that comes the following
\autoref{th:sizeSq}.
\begin{restatable}{thm}{samples}\label{th:sizeSq} Let $\CC$ be a $q$-qubit IQP,
    fix $\epsilon > 0$ and let $\Ng$, $\Nk$ the number of samples required to
    estimate $\braket{0^{\otimes q} | \CC | 0^{\otimes q}}$ using the graph
    encoding and the nonadaptive KLM scheme respectively. Then we can write 
    $
        {\Ng = \alpha(\CC) \Nk,}
    $
    and, for large enough $q$, we have
    $
        \pr{\alpha(\CC) < 1} \approx 1.
    $
\end{restatable}


This theorem is discussed and proved in \autoref{sec:postSelectionRate}.
Similarly, in \autoref{sec:photons}, we show the following \autoref{th:sizePq}.
\begin{restatable}{thm}{photons}\label{th:sizePq} Let $P_q$ be the set of $q$-qubit
    IQP circuits for which the estimation of the zero-zero probability via the
    graph encoding technique requires fewer photons per shot. Then, 
    \begin{equation}
        \lim_{q \to \infty} \frac{\abs{P_q}}{\abs{\II_q}} = 1.
    \end{equation}
\end{restatable}
Both theorems are proved by combinatorial arguments.




==> sections/iqp.tex <==

\section{IQP circuits}\label{sec:iqp}

The \emph{Instantaneous Quantum Polynomial} (IQP) circuits form a restricted
model of quantum computation. They were introduced in
\cite{shepherd_temporally_2009} as a subset of quantum circuits that is rich
enough to enable sampling from distributions that is hard to describe
classically. A $q$-qubit IQP circuit has the following structure. On input
$\ket{0^{\otimes q}}$ apply $H^{\otimes q}$, then a circuit $\mathcal D$
diagonal in the Z-basis and another layer of Hadamard; finally measure in the
Z-basis and obtain $q$-bit string $y$. In a more concise way, an IQP circuit
$\mathcal C$ can be written $\mathcal C = H^{\otimes q} \mathcal D H^{\otimes
q}$ (we may specify the number of qubits by writing $\CC_q$). It is shown under
usual complexity assumptions in \cite{bremner_average-case_2016} that sampling
from the output distribution of IQP circuits built from 2-qubit and 3-qubit gate
sets with small multiplicative error is hard classically. The nice structure of
IQP circuits combined with the hardness result regarding their classical
simulation motivate the study of their encoding into graphs.

We shall call a subcircuit of the form $\mathcal D H^{\otimes q}$ a
\emph{layer}, and use the following more general construction of IQP-$l$
circuits, that are circuits of the form
\begin{equation}
\CC = H^{\otimes q} \prod_{i=1}^l \left(\mathcal D_i H^{\otimes q}\right) ,
\end{equation}
where the $\mathcal D_i$'s are random circuits that are diagonal in the Z-basis.
It is shown in \cite{havlicek_supervised_2019} that it is possible to compute
elements of the output distribution of IQP-1 circuits up to polynomially-small
additive error in classical polynomial time, while the same task is intractable
for IQP-2 circuits with the same classical method.
% Thanks to this hardness
% result, the authors use IQP circuits in quantum machine learning as a
% classically-hard-to-estimate feature map for solving classification problems.
Taking inspiration from the seminal work of \cite{dawson_quantum_2004}, which
introduced the \emph{sum over paths} description
(\autoref{eq:amplitudeSumValidAssigment}) of quantum circuits, it has been shown
in \cite{bremner_average-case_2016} that the amplitudes of \{H, Z, CZ, CCZ\}
circuits can be expressed in the same fashion. More precisely, let $\CC$ be an
IQP-1 circuit over $q$ qubits. The authors show that there exists a polynomial
$f$ over sufficiently many binary variables $x_1, \cdots, x_n$ of the form
\begin{equation}\label{eq:polynomialIQP}
    f(\x) = \sum_{i, j, k}\alpha_{ijk}x_ix_jx_k + \sum_{i, j}\beta_{ij}x_ix_j + \sum_{i}\gamma_{i}x_i ,
\end{equation}
where $\alpha_{ijk}, \,\beta_{ij}, \, \gamma_{i} \in \{0, 1\}$, such that
\begin{equation}
\braket{0^{\otimes q} | \CC | 0^{\otimes q}} = \frac{1}{2^q} \sum_{x \in \{0, 1\}^n}(-1)^{f(x)}.
\end{equation}
From a polynomial, its associated circuit is constructed by applying a Z, CZ or
CCZ gate involving qubits $i$, $j$ and/or $k$ whenever $\gamma_i, \beta_{ij},
\alpha_{ijk}=1$ respectively, and vice versa. The extension to IQP-$l$ circuits
for arbitrary $l$ is straightforward.

We call the amplitude $\braket{0^{\otimes q} | \CC | 0^{\otimes q}}$ the
\emph{zero-zero} amplitude of $\CC$ (and its squared modulus the
\emph{zero-zero} probability). Remark that the diagonal part is built upon the
phase gates described in \autoref{eq:defPhaseGates} with $\theta = \pi$. As a
matter of fact, we already have for free the mapping of family of IQP circuits
to graph but at the expense of using the redundant Hadamard gates imposed in the
encoding of \cite{dawson_quantum_2004}. They are necessary to bound the degree
of the polynomial to which the circuit is associated, as otherwise that
polynomial would not have constant but linear in the number of succeeding
Toffoli gates degree. The large overhead in the total number of gates in the
circuit and hence in the size of the resulting graph cannot be dealt with
easily. This is because from the permanent's point of view, there is no way of
expressing the identity $H^2 = \id\ $ and for that reason, those redundant
Hadamard gates make the permanent superfluously harder to compute. Also, the
supplementary Hadamard impose a specific structure for the the polynomial: if a
variable appears in a cubic clause, then it appears in exactly two quadratic
clauses. This structure relaxes the constraints for designing a cubic clause
gadget as it does not have to deal with \autoref{ob:zero}. That is why the cubic
clause gadget designed in \cite{rudolph_simple_2009} is not a generic clause
gadget. Finally, as the polynomial associated to IQP circuits is already bounded
by 3 by construction, the redundant Hadamard gates become even more superfluous.
This motivates the design of a \emph{standalone} gadget for the cubic clauses
that fulfills the conditions imposed on the quadratic clause gadget. In this
work, an encoding of IQP circuits amplitudes is derived by 
\begin{itemize}[label=--]
    \item first designing a gadget for
each phase gate of \autoref{eq:defPhaseGates},
    \item then setting $\theta = \pi$,
    \item and finally construct a graph from the circuit using the gadgets as per
\cite{rudolph_simple_2009}.
\end{itemize}
We denote by $A_i(\theta)$ the gate encoding the amplitudes of the $P_i(\theta)$
gate. The $i+1$ first rows/columns index the outer vertices of the gadget, while
the remaining ones indicate the inner vertices. The following gadgets are
derived by solving the system of equations returned by \autoref{alg:generation}
on the appropriate parameters. The adjacency matrix $A_i(\theta)$ is that of a
clause of degree $i$ with coefficient $\theta$. The degree-one monomials with
coefficient $\theta$ are encoded into the following gadget:
\begin{equation*}
A_2(\theta) := \begin{bmatrix}
    e^{i\theta}
\end{bmatrix}.
\end{equation*}

$P_1(\theta)$ amplitudes are encoded into a gadget with one inner vertex:
\begin{equation*}
A_3(\theta) :=\begin{bmatrix}\frac{1}{2}(1+e^{i \theta}) & \frac{1}{2}(e^{i
    \theta} - 1) & \frac{1}{2}(1 - e^{i \theta})\\-1 & 0 & 1\\1 & 1 &
    1\end{bmatrix}.
\end{equation*}
Remark that letting $\theta = \pi$ yields the gadget encoding the quadratic
clauses of \cite{rudolph_simple_2009}, which is consistent with the observation
that both Hadamard (regardless its rescaling factor) and CZ amplitudes are of
the form $(-1)^{xy}$ for the suitable choice of variables $x$ and $y$.

Finally, $P_2(\theta)$ amplitudes are encoded into the following gadget
comprising two inner vertices. Let $\eta(\theta) := \frac{1}{6}\sqrt{3 (1+i)(1
- e^{i \theta})}$,
% \resizebox{0.5\textwidth}{!}{
\begin{equation*}
% \hspace{-.5cm}
A_3(\theta) :=
\begingroup 
\setlength\arraycolsep{1pt}
\begin{bmatrix}
    \frac{e^{i \theta} - (1 + 12 i)}{-12 i}
    & -\eta(\theta)
    & -\eta(\theta)
    &  \frac{\eta(\theta)}{\sqrt{2}} e^{i \frac \pi 4}
    &  \frac{-\eta(\theta)}{\sqrt{2}}
\\  -\eta(\theta)
    & i
    & -1 +i
    & 1
    & e^{i \frac{3\pi}{4}}
\\ -\eta(\theta)
    & -1 +i
    &i
    & 1
    & e^{i \frac{3\pi}{4}}
\\ \frac{\eta(\theta)}{\sqrt{2}} e^{i \frac \pi 4}
    & 1
    & 1
    & 1
    & 0
\\- \sqrt{ \frac{\left(1 -e^{i \theta}\right)}{24(1+i)}}
    & e^{i \frac{3\pi}{4}}
    & e^{i \frac{3\pi}{4}}
    & 0
    & 1
\end{bmatrix}.
\endgroup
\end{equation*}
% }

Foremost, for each gadget the number of inner vertices is minimal according to
\autoref{eq:optimalK}.

With these three gadgets in hand, the graph encoding of $q$-qubit IQP circuits
is characterized by the following \autoref{pr:numberOfNodes}. Throughout rest,
let $\#(\UU)$ denote the number of occurrences of the gate $\UU$ in the circuit
$\CC$, \eg $\#(H) = 2q$.

\begin{proposition}\label{pr:numberOfNodes} Let $\CC$ be a $q$-qubit IQP circuit
    of depth $d$ and $\GG_\CC$ be the graph such that ${\braket{0^{\otimes{q}} |
    \CC | 0^{\otimes{q}}} = \frac{1}{2^q}\per{\GG_\CC}}$. Then,
    $\GG_\CC$ is a graph comprising the following number of nodes: 
    \begin{equation} M = q + \#(P_0(\theta)) +
    3\#(P_1(\theta)) + 5\#(P_2(\theta)). 
    \end{equation}
\end{proposition}
\begin{proof}
    The proof simply follows from counting the number of nodes of each gadget.
\end{proof}
\noindent Note that ${M =\bigo{qd}}$. Conversely, the encoding of
\cite{rudolph_simple_2009} induces a graph with
\begin{equation}
2q + \#(P_0(\theta)) + 3 \#(P_1(\theta)) + 9\#(P_2(\theta))
\end{equation}
nodes. This is indeed asymptotically the same order of magnitude, but the
difference is noticeable on small size experiments and especially if one tries
to implement it on near-term devices. A detailed walkthrough of the encoding of
an IQP circuit's zero-zero amplitude onto a graph using our findings is given in
\autoref{sec:example}.

\input{sections/subsections/iqp/applications}

\input{sections/subsections/iqp/example}




==> sections/short_abstract.tex <==
\pagenumbering{gobble}

\begin{localsize}{11}
\section*{Short Abstract}


In this work, we propose a general method for computing exponential sums of
$\mathbb F_2$-valued polynomials with complex coefficients as a matrix
permanent. That is, from a $n$-variable polynomial $f$ with binary variables
and complex coefficients, we show how to construct a graph $G$ with adjacency matrix $\mathcal G$ such that
$$
  \sum_{x \in \{0, 1\}^n} e^{i f(\x)} = \per{\mathcal G},
$$
in time polynomial in the number of clauses of $f$. This is achieved by going
beyond existing work on links between matrix permanents and sum of polynomial
evaluation, which were only applicable to a very limited class of polynomials.
This encoding proves useful in quantum computation. In the context of
circuit-based quantum computation, such sums arise as a product of the
\emph{sum-over-paths} interpretation of quantum probability amplitudes. On the
other hand, the matrix permanent is a combinatorial object that finds use in
photonic quantum computing as the way to describe probability amplitudes. We aim
to find links between these two seemingly different models of quantum
computation. 

A discrete version of Feynman's path integral, the \emph{sum-over-paths}
interpretation, is a powerful tool in quantum computation. It allows one to
express the transition amplitude from the computational basis state $\ket{\bs
a}$ to the computational basis state $\ket{\bs b}$ as $\braket{\bs b | \CC | \bs
a} \propto \sum_{\bs x \in \{0, 1\}^v} e^{i f(\bs x)}$, where $f$ is a $\mathbb
F_2$-valued polynomial with complex coefficients and $v$ is the number of qubits
in the circuit plus the number of gates creating coherence in the circuit (\eg
Hadamard gates). Conversely, the quantum probability amplitudes resulting from a
linear optical computation are -- for input and output occupancy $\bs s = (s_1,
\cdots, s_m)$ and $\bs t = (t_1, \cdots, t_m)$, where $s_i$ (resp. $t_i$) is the
number of photons in input (resp. output) mode $i$, and a unitary matrix
$\mathcal U \in SU(m)$ -- of the form $\braket{\bs t | \mathcal U |\bs u}
\propto \per{\mathcal U_{\bs s, \bs t}}$. Provided a quantum circuit $\CC$ and
its associated polynomial $f$ resulting from the sum-over-paths interpretation
of the amplitude $\braket{\bs b | \CC | \bs a}$, we use our encoding to
construct a graph $G$ such that $$\braket{\a | \mathcal C | \b } \propto
\per{\mathcal G}.$$ We are in turn able to construct a linear optical circuit $\mathcal V$
such that $$\braket{\bs 1_n | \mathcal V |\bs 1_n} \propto \braket{\bs b | \CC |
\bs a },$$ where  $\ket{\bs 1_n} =\ket{1^{\otimes n}0^{\otimes{m-n}}}$, using
earlier work on graph-problems solving in linear optics to map (a rescaled
version of) $G$ to a unitary matrix $\mathcal V$. By providing yet another way
to map gate-based quantum circuit to linear optical circuits, our method
 strengthens the connection between circuit-based and photonic quantum
computation, as one can use a photonic device to compute an estimate of a matrix
permanent. This encoding opens the door to a whole new family of classical
algorithms for the simulation of quantum circuits based on permanent estimation.

Second, the encoding we provide is benchmarked against the nonadaptive
Knill-Laflamme-Milburn (KLM) implementation of universal linear optical quantum
computation on the task of estimating an output probability of Instantaneous
Quantum Polynomial-time (IQP). While both techniques indeed require
exponentially many samples to provide an estimate within small additive error,
we show that the graph encoding we derived requires both fewer samples to reach
the same accuracy as KLM and fewer single photons per shot for almost all
instances.

\end{localsize}


\newpage
\pagenumbering{arabic}

==> sections/subsections/benchmark/boosting.tex <==
\subsection{Probability boosting}\label{sec:boosting}

In \cite{mezher_solving_2023}, the authors present a probability boosting
technique which allows a better approximation of the permanent with fewer
samples.

Let $A$ be such an $M \times M$ matrix. The technique relies on modified
adjacency matrix
\begin{equation}
A_{\varepsilon} =  A + \varepsilon \id_{M\times M},
\end{equation}
where $\varepsilon \in \mathbb R^+$. The idea is to get rought estimates of the
permanent of $A_{\varepsilon}$ for $M+1$ differents values of $\varepsilon$,
from which one is able to recover the permanent of $A$ by solving a system of
linear equations to which $\per{A}$ is an entry of a solution. Indeed for large
enough $\varepsilon$, $\abs{\per{A_\varepsilon}} > \abs{\per{A}}$, indicating
that the permanent of $A_\varepsilon$ can be estimated from fewer samples. The
technique was introduced for real-valued matrices.  We show herein that
probability boosting techinque of \cite{mezher_solving_2023} can be applied to
the class of matrices which are adjacency matrices of graphs encoding the IQP
circuits zero-zero amplitudes.


First, we shall prove the following proposition.
\begin{proposition}
    Let $\CC$ be a $q$-qubit IQP circuit, and let $A$ be the $M \times M$
    adjacency matrix of $\GG_\CC$. Then,
    \begin{equation}
   1+\varepsilon \leq \|A_\varepsilon\|_2 \leq \| A \|_\infty + \varepsilon.
    \end{equation}
\end{proposition}
\begin{proof}
    The lower bound is follows from Cauchy's interlacing theorem for singular values
    \cite{thompson_principal_1972} applied to $A_\varepsilon$.

    In the graph we consider, $\|A\|_1 = \|A\|_\infty$, since all gadgets are
    symmetric and there is exactly one 1 in a row/column corresponding to the
    outer verticesn the rest of the entries are zeros, and only zeros in that of
    the inner vertices. Then, the upper bound is found as follows:
    \begin{equation}
    \begin{aligned}
       \|A_\varepsilon\|^2_2
        = \rho(A_\varepsilon^* A_\varepsilon) 
        \leq \| A_\varepsilon^* A_\varepsilon \|_\infty 
        \leq \| A_\varepsilon^* \|_\infty \| A_\varepsilon \|_\infty 
        = \| A_\varepsilon\|_1 \| A_\varepsilon \|_\infty 

        \leq (\| A \|_\infty + \varepsilon)^2,
    \end{aligned}
    \end{equation}
    the results follows by taking the square root of both sides.
\end{proof}
This implies, similarly, that $\|A_\varepsilon\|_2 = \bigo{\varepsilon}$ and
$\per{A_\varepsilon} = O(\varepsilon^M)$ when $\varepsilon \rightarrow \infty$ and $M$ is
fixed.

Using the permanent-of-sums formula, we can write
\begin{equation}
\per{A_\varepsilon} = \sum_{i=0}^M c_i \varepsilon^i,
\end{equation}
with $c_0 = \per A$, $c_M = \per{\id} = 1$ and $c_i$ is the sum of permanents of
$(M-i) \times (M-i)$ submatrices of $A$. Notice that sampling the linear optical
interferometer onto which $A_\varepsilon$ is encoded gives an estimate of
$\abs{\per{A_\varepsilon}}^2$, hence we write
\begin{equation}
\abs{\per{A_\varepsilon}}^2 = \abs{\sum_{i=0}^M c_i \varepsilon^i}^2,
    % = c_0^2 + \varepsilon c_0 c_1 + \varepsilon c_0 \bar{c_1} + \ldots + \varepsilon^{2i} \abs{c_i}^2+ \ldots +\varepsilon^{2M} \abs{c_M}^2,
\end{equation}
where, in our case as well, $c_0$ is real. We linearize the polynomial by
defining $y_k := c_i\bar{c_j}$ (for some irrelevant \emph{naming map} $(c_i,
\bar{c_j}) \mapsto k$) and set ${y_i := \abs{c_i}^2}$ for ${i = 0, \ldots, M}$
for simplicity. Then, an estimate of $\abs{\per{A}}^2$ is obtained by computing
$M$ estimates of $\abs{\per{A_{\varepsilon}}}^2$ for $M$ randomly chosen
$\varepsilon$'s. This procedure yields the following system
\begin{equation}
\begin{cases}
   \abs{\sum_{i=0}^M c_i \varepsilon_1^i}^2 = & \abs{\per{A_{\varepsilon_1}}}^2 \\
   \abs{\sum_{i=0}^M c_i \varepsilon_2^i}^2 = & \abs{\per{A_{\varepsilon_2}}}^2 \\
   \ \qquad \vdots & \qquad \vdots \\
   \abs{\sum_{i=0}^M c_i \varepsilon_M^i}^2 =& \abs{\per{A_{\varepsilon_M}}}^2 \\
\end{cases}.
\end{equation}


We linearize the polynomials to obtain polynomials of degree $2M$ in the unknown
$y_i$'s. Define the matrices $\mathcal E_1$ and $\mathcal E_2$ as follows.
\begin{equation}
   \mathcal E_1 :=
   \begin{pmatrix}
        1 & \varepsilon_1^2 & \varepsilon_1^4 &  \cdots & \varepsilon_1^{2M}            \\
    1 & \varepsilon_2^2 & \varepsilon_2^4 & \cdots & \varepsilon_2^{2M}             \\
    \vdots & \vdots & \vdots & \ddots & \vdots                             \\
    1 & \varepsilon_{M+1}^2 & \varepsilon_{M+1}^4 & \cdots & \varepsilon_{M+1}^{2M}
\end{pmatrix}.
\end{equation}
and $\mathcal E_2$ contains suitable powers of $\varepsilon$. Let ${\mathcal{E} :=
\begin{pmatrix} \mathcal E_1 & \mathcal E_2 \end{pmatrix}}$
constructed by stacking $\mathcal E_1$ and $\mathcal E_2$ horizontally.
For simplicity, consider the vector of variables
$\bs y := \begin{pmatrix}
    y_0 &
    y_1 &
    \cdots &
\end{pmatrix}$ where the first $M$ entries are the $y_i = \abs{c_i}^2$. We
then write the system in matrix form
\begin{equation}
\mathcal E
\bs y^T
=
\begin{pmatrix}
    \abs{\per{A_{\varepsilon_1}}}^2 \\
    \abs{\per{A_{\varepsilon_2}}}^2 \\
    \vdots \\
    \abs{\per{A_{\varepsilon_M}}}^2\\
\end{pmatrix}.
\end{equation}


$\mathcal E_1$ is a Vandermonde matrix, as the $\varepsilon_i$'s are chosen
different from one another. Hence, we compute the reduced echelon form of the
system and obtain parametrized solutions for $y_0, \ldots, y_M$. Notice that
$y_i = f_i(\mathcal Y)$ for some linear function $f$, and in particular ${f_0(0)
= y_0 = |\per{A}|^2}$. To conclude, the probability boosting technique also
applies to adjacency matrices of the graphs encoding the zero-zero probability
of $q$-qubit IQP circuits. With this technique in hand, the almost-unit
probability plateau of \autoref{fig:prAlphaLessThanOne} could be reached at
smaller values of $q$, further improving the efficiency of the scheme.

==> sections/subsections/iqp/applications.tex <==
\subsection{Applications}

Despite their non-universality, IQP circuits find use in several domains. First,
a striking result from \cite{havlicek_supervised_2019} relies on the hardness of
estimating output probabilities of IQP-2 circuits via classical methods. The
authors showcase the use of IQP circuits to build a hard-to-simulate feature map
for solving classification problems.

The $P_i(\theta)$ gates also find use outside the scope of IQP circuits. For
instance, such gates can be used to implement diagonal logical gates, as shown
in \cite{hu_climbing_2021}, where the authors describe how to construct a CSS
code that realizes a diagonal gate at the $l$-th level of the Clifford hierarchy
from a CCS code using, among other things, $P_l(\theta)$ gates. Logical diagonal
gates are crucial to implement error-corrected quantum algorithm, \eg the
quantum Fourier transform \cite{coppersmith_approximate_2002} which is used in
the period finding routine of Shor's algorithm \cite{shor_polynomial-time_1997}
heavily relies on phase gates.
